ExACT: Teaching AI Agents to Explore with Reflective-MCTS and Exploratory Learning

Autonomous agents have demonstrated significant potential in automating complex multistep decision-making tasks. However, even state-of-the-art vision-language models (VLMs), such as GPT-4o, still fall short of human-level performance, particularly in intricate web environments and long-horizon tasks. To address these limitations, we present ExACT, an approach to combine test-time search and self-learning to build o1-like models for agentic applications. We first introduce Reflective Monte Carlo Tree Search (R-MCTS), a novel test time algorithm designed to enhance AI agents' ability to explore decision space on the fly. R-MCTS extends traditional MCTS by 1) incorporating contrastive reflection, allowing agents to learn from past interactions and dynamically improve their search efficiency; and 2) using multi-agent debate for reliable state evaluation. Next, we introduce Exploratory Learning, a novel learning strategy to teach agents to search at inference time without relying on any external search algorithms. On the challenging VisualWebArena benchmark, our GPT-4o based R-MCTS agent achieves a 6% to 30% relative improvement across various tasks compared to the previous state-of-the-art. Additionally, we show that the knowledge and experience gained from test-time search can be effectively transferred back to GPT-4o via fine-tuning. After Exploratory Learning, GPT-4o 1) demonstrates the ability to explore the environment, evaluate a state, and backtrack to viable ones when it detects that the current state cannot lead to success, and 2) matches 87% of R-MCTS's performance while using significantly less compute. Notably, our work demonstrates the compute scaling properties in both training - data collection with R-MCTS - and testing time. These results suggest a promising research direction to enhance VLMs' capabilities for agentic applications via test-time search and self-learning.

==> floats/table_learning.tex <==
\begin{table}
  \centering
  \scalebox{0.95}{
  \begin{tabular}{lcc c cccc}
    \toprule
    % out of 0-75 tasks for the classifields subtask
    \multirow{2}{*}{Method} & \multirow{2}{*}{Model} & \multirow{2}{*}{Max Steps} & \multirow{2}{*}{Training} & \multirow{2}{*}{Tokens} & \multicolumn{3}{c}{Success} \\
    \cmidrule{6-8}
    & & & & & Seen & Unseen & Overall \\
    \midrule
    % ReACT & GPT-4o & 1.0x & 52/71 & 0/163 & 22.2\%\\
    % 128k / 0.9k
    \react{} & GPT-4o-mini & 20 & \xmark & 1.0x & - & - & 20.9\%\\
    % 110k / 20k
    \react{} & o1-mini & 20 & \xmark & 1.0x$^\dagger$ & - & - & 23.9\%\\
    \midrule
    % 56k
    \react{} & GPT-4o & 5 & \xmark & 1.0x & - & - & 22.2\%\\
    % 133k / 0.8k  % note that react uses more token as max step is larger for all runs in this table
    \react{} & GPT-4o & 20 & \xmark & 2.4x & - & - & 22.2\%\\
    % 75/234 % sft used much less because these are filtered due to intermediate steps
    % 540k/51k
    \rmctsdebate{} & GPT-4o & 20 & \xmark & 9.6x & - & - & 32.1\%\\
    \midrule
    % 328k / 0.8k
    % ReACT & GPT-4o-sft-v4 & 2.5x & 50/71 & 16/163 & 28.2\%\\
    % ReACT & Chain-SFT & 2.5x & 50/71 & 16/163 & 28.2\%\\
    % 319k / 0.8k
    % ReACT & GPT-4o-sft-v5 & 2.4x & 52/71 & 16/163 & 29.1\%\\
    % ReACT & Chain-SFT & 2.4x & 52/71 & 16/163 & 29.1\%\\
    % ReACT & GPT-4o-sft-v7 & 2.4x & 52/65 & 21/169 & 31.2\%\\
    % 158k / 0.8k
    % ReACT & Chain-SFT & 65 & 1.2x & 52/65 & 21/169 & 31.2\%\\
    \react{} & \chainsftshort{} & 20 & 65 & 2.5x & 80.0\% & 12.4\% & 31.2\%\\
    % 210k
    % ReACT & GPT-4o-tree-sft-v1 & 1.6x & 31/39 & 35/195 & 28.2\%\\
    % ReACT & Tree-SFT-v1 & 39 & 1.6x & 31/39 & 35/195 & 28.2\%\\
    % ReACT & Tree-SFT-v1 & 39 & 3.7x & 79.5\% & 17.9\% & 28.2\%\\
    % data/visualwebarena/eval_results/cot/gpt-4o_treesftv9_v6.2_20steps_classifields_all
    % seen 28/35, unseen 37/199
    % 203k / 1.7k
    \react{} & \treesftshort{} & 20 & 35 & 3.6x & 80.0\% & 18.6\% & 27.8\%\\
    \bottomrule
  \end{tabular}
  }
  \caption{Comparing different model's performance evaluated in the Classifieds environment. Since GPT-4o finetuning does not support images, we run all experiments in a text-only modality provided by VisualWebArena. \change{``Training" indicates whether the model has undergone training in \Cref{subsec:Learning}, and if so, how many trajectories are used.} $^\dagger$While total token consumption is similar, o1-mini used 20x more output tokens (reasoning + output) than GPT-4o-mini's output tokens (output).
  }
  \label{tbl:gpt4o_tuning}
\end{table}

==> floats/table_main.tex <==
% \begin{table}[ht!]
%   \centering
%   \begin{tabular}{ll cc cc cc}
%     \toprule
%     \multirow{2}{*}{Method} & \multirow{2}{*}{Search} & 
%     \multicolumn{2}{c}{Classifieds} & \multicolumn{2}{c}{Reddit} & \multicolumn{2}{c}{Shopping} \\
%     \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
%     & & Tokens & Success & Tokens & Success & Tokens & Success\\
%     \midrule
%     % data/visualwebarena/eval_results/cot_som/gpt-4o_v6.1_classifields_80_tsubset
%     % 53.8k/0.40k
%     \react{} & - 
%     & 1x & 28.6\%
%     % data/visualwebarena/eval_results/cot_som/gpt-4o_v6_reddit_80_tsubset
%     % 39.3k/0.48k
%     & 1x & 13.8\%
%     % data/visualwebarena/eval_results/cot_som/gpt-4o_v6.1_shopping_120_tsubset
%     % data/visualwebarena/eval_results/cot_som/gpt-4o_v6.1_shopping_0-465
%     % 66.0k/0.46k
%     & 1x & 23.2\%\\
%     % ToT$_{\textrm{BFS}}$ & BFS
%     \tot{} & BFS
%     % data/visualwebarena/eval_results/tot_som/gpt-4o_v6.1cached_bfs_vrubric_classifields_80_tsubset
%     % 151.1k/26.2k
%     & 3.2x & 30.7\% 
%     & 4.7x & 19.5\% 
%     % data/visualwebarena/eval_results/tot_som/gpt-4o_v6.1cached_vrubric_shopping_120_tsubset
%     % 195.8k/31.3k
%     & 4.3x & 29.2\% \\
%     % ToT$_{\textrm{DFS}}$ & DFS
%     \tot{} & DFS
%     & 3.1x & 30.3\% 
%     % 148k/20.6k
%     & 4.2x & 16.7\% 
%     & 4.0x & 28.3\% \\
%     % Search Agent & A-star 
%     \searchagent & Best-First
%     % data/visualwebarena/eval_results/searchagent_som/gpt-4o_v6.1cached_classifields_80_tsubset
%     & 4.2x & 33.8\%
%     & 5.4x & 21.9\%
%     & 5.1x & 30.3\%\\
%     % mcts above + the prompt changes used in rmcts_v7.2
%     \mcts{} & MCTS 
%     % 350k/35k
%     & 7.2x & 37.6\%
%     & 9.5x & 23.8\% %
%     & 8.9x & 29.4\% \\%
%     \midrule
%     % reinforced policy + reinforced rubric value function
%     % +some policy prompt fixing25_classifields_0-75
%     \rmcts{} & MCTS 
%     % data/visualwebarena/eval_results/rmcts_som/gpt-4o_v7.2cached_refl3_vrubric_classifields_80_tsubset
%     % 332k/50k
%     & 7.3x & 40.2\%
%     % 300k/34k
%     & 7.3x & 25.2\%
%     % 332k/45k
%     & 7.6x & 31.9\%
%     \\
%     % reinforced policy + reinforced debate value function
%     \rmctsdebate{} & MCTS 
%     % data/visualwebarena/eval_results/rmcts_som/gpt-4o_v7.4.1cached_refl3_vredebate_trhld0.5_classifields_80_tsubset
%     % 373.6k/34.0k
%     & 7.4x & \textbf{41.0}\%
%     % data/visualwebarena/eval_results/rmcts_som/gpt-4o_v7.4.1cached_refl3_vredebate_trhld0.5_reddit_80_tsubset
%     % 560k/37.7k
%     & 9.7x & \textbf{28.7}\%
%     % 674k/49.5k
%     & 10.1x & \textbf{32.3}\%
%     \\
%     \bottomrule
%   \end{tabular}
%   \caption{Comparing different agent's token consumption and performance on VisualWebArena. We show average token used per task using \react{} as a baseline.}
%   \label{tbl:main_vwa}
% \end{table}
\begin{table}[t!]
  \centering
  \scalebox{0.92}{
  \begin{tabular}{lc ccc cc cc}
    \toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Search} & \multirow{2}{*}{Value} & 
    \multicolumn{2}{c}{Classifieds} & \multicolumn{2}{c}{Reddit} & \multicolumn{2}{c}{Shopping} \\
    \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    & & & Tokens & Success & Tokens & Success & Tokens & Success\\
    \midrule
    % data/visualwebarena/eval_results/cot_som/gpt-4o_v6.1_classifields_80_tsubset
    % 53.8k/0.40k
    \react{} & - & -
    & 1x & 28.6\%
    % data/visualwebarena/eval_results/cot_som/gpt-4o_v6_reddit_80_tsubset
    % 39.3k/0.48k
    & 1x & 13.8\%
    % data/visualwebarena/eval_results/cot_som/gpt-4o_v6.1_shopping_120_tsubset
    % data/visualwebarena/eval_results/cot_som/gpt-4o_v6.1_shopping_0-465
    % 66.0k/0.46k
    & 1x & 23.2\%\\
    % ToT$_{\textrm{BFS}}$ & BFS
    \tot{} & BFS & $\texttt{SA}$
    % data/visualwebarena/eval_results/tot_som/gpt-4o_v6.1cached_bfs_vrubric_classifields_80_tsubset
    % 151.1k/26.2k
    & 3.2x & 30.7\% 
    & 4.7x & 19.5\% 
    % data/visualwebarena/eval_results/tot_som/gpt-4o_v6.1cached_vrubric_shopping_120_tsubset
    % 195.8k/31.3k
    & 4.3x & 29.2\% \\
    % ToT$_{\textrm{DFS}}$ & DFS
    \tot{} & DFS & $\texttt{SA}$
    & 3.1x & 30.3\% 
    % 148k/20.6k
    & 4.2x & 16.7\% 
    & 4.0x & 28.3\% \\
    % Search Agent & A-star 
    \searchagent & Best-First & $\texttt{SA}$
    % data/visualwebarena/eval_results/searchagent_som/gpt-4o_v6.1cached_classifields_80_tsubset
    & 4.2x & 33.8\%
    & 5.4x & 21.9\%
    & 5.1x & 30.3\%\\
    % mcts above + the prompt changes used in rmcts_v7.2
    \mcts{} & MCTS & $\texttt{SA}$
    % 350k/35k
    & 7.2x & 37.6\%
    & 9.5x & 23.8\% %
    & 8.9x & 29.4\% \\%
    \midrule
    % reinforced policy + reinforced rubric value function
    % +some policy prompt fixing25_classifields_0-75
    \rmcts{} & MCTS & $\texttt{SA}$
    % data/visualwebarena/eval_results/rmcts_som/gpt-4o_v7.2cached_refl3_vrubric_classifields_80_tsubset
    % 332k/50k
    & 7.3x & 40.2\%
    % 300k/34k
    & 7.3x & 25.2\%
    % 332k/45k
    & 7.6x & 31.9\%
    \\
    % reinforced policy + reinforced debate value function
    \rmcts{} & MCTS  & $\texttt{MAD}$
    % data/visualwebarena/eval_results/rmcts_som/gpt-4o_v7.4.1cached_refl3_vredebate_trhld0.5_classifields_80_tsubset
    % 373.6k/34.0k
    & 7.4x & \textbf{41.0}\%
    % data/visualwebarena/eval_results/rmcts_som/gpt-4o_v7.4.1cached_refl3_vredebate_trhld0.5_reddit_80_tsubset
    % 560k/37.7k
    & 9.7x & \textbf{28.7}\%
    % 674k/49.5k
    & 10.1x & \textbf{32.3}\%
    \\
    \bottomrule
  \end{tabular}
  }
  \caption{Comparing different agent's token consumption and performance on VisualWebArena. We show average token used per task using \react{} as a baseline.}
  \label{tbl:main_vwa}
\end{table}

==> floats/table_main_ARR_oct.tex <==
\begin{table}[t!]
  \centering
  \scalebox{0.75}{
  \begin{tabular}{lc cc cc cc cc}
    \toprule
    \multirow{2}{*}{Search}  & \multirow{2}{*}{Value} & 
    \multicolumn{2}{c}{Classifieds (VWA)} & \multicolumn{2}{c}{Reddit (VWA)}& \multicolumn{2}{c}{Shopping (VWA)}& \multicolumn{2}{c}{\change{GitLab (WA)}}\\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
    & & Tokens & Success & Tokens & Success & Tokens & Success & \change{Tokens} & \change{Success}\\
    \midrule
    \xmark \, (\react{}) & -
    & 1x & 28.6\% \tiny{\change{($\pm$0.9\%)}}
    & 1x & 13.8\% \tiny{\change{($\pm$0.9\%)}}
    & 1x & 23.2\% \tiny{\change{($\pm$0.7\%)}}
    & \change{1x} & \change{11.3\%} \tiny{\change{($\pm$1.1\%)}}
    \\
    \tot{}$_\texttt{BFS}$ & $\texttt{SA}$
    & 3.2x & 30.7\% \tiny{\change{($\pm$0.9\%)}}
    & 4.7x & 19.5\% \tiny{\change{($\pm$0.9\%)}}
    & 4.3x & 29.2\% \tiny{\change{($\pm$0.8\%)}}
    & \change{4.6x} & \change{14.1\%} \tiny{\change{($\pm$1.0\%)}}
    \\
    \tot{}$_\texttt{DFS}$ & $\texttt{SA}$
    & 3.1x & 30.3\% \tiny{\change{($\pm$0.7\%)}}
    & 4.2x & 16.7\% \tiny{\change{($\pm$1.2\%)}}
    & 4.0x & 28.3\% \tiny{\change{($\pm$0.9\%)}}
    & \change{4.3x} & \change{14.1\%} \tiny{\change{($\pm$1.0\%)}}
    \\
    \searchagent{} & $\texttt{SA}$
    & 4.2x & 33.8\% \tiny{\change{($\pm$1.0\%)}}
    & 5.4x & 21.9\% \tiny{\change{($\pm$1.2\%)}}
    & 5.1x & 30.3\% \tiny{\change{($\pm$0.8\%)}}
    & \change{3.0x} & \change{13.8\%} \tiny{\change{($\pm$1.7\%)}}
    \\
    MCTS & $\texttt{SA}$
    & 7.2x & 37.6\% \tiny{\change{($\pm$1.1\%)}}
    & 9.5x & 23.8\% \tiny{\change{($\pm$1.4\%)}}
    & 8.9x & 29.4\% \tiny{\change{($\pm$0.7\%)}}
    & \change{5.7x} & \change{19.9\%} \tiny{\change{($\pm$1.7\%)}}
    \\
    \midrule
    \rmcts{} & $\texttt{SA}$
    & 7.3x & 40.2\% \tiny{\change{($\pm$0.7\%)}}
    & 7.3x & 25.2\% \tiny{\change{($\pm$1.3\%)}}
    & 7.6x & 31.9\% \tiny{\change{($\pm$0.7\%)}}
    & \change{6.0x} & \change{20.9\%} \tiny{\change{($\pm$1.9\%)}}
    \\
    \rmcts{}  & $\texttt{MAD}$
    & 7.4x & \textbf{41.0}\% \tiny{\change{($\pm$0.9\%)}}
    & 9.7x & \textbf{28.7}\% \tiny{\change{($\pm$1.4\%)}}
    & 10.1x & \textbf{32.3}\% \tiny{\change{($\pm$0.7\%)}}
    & \change{8.8x} & \change{\textbf{23.5}\%} \tiny{\change{($\pm$1.3\%)}}
    \\
    \bottomrule
  \end{tabular}
  }
  \caption{Comparing different agent's token consumption and performance on VisualWebArena \change{(VWA) as well as on the GitLab domain from WebArena (WA)}. We show average token used per task using \react{} as a baseline. \change{We adopt the bootstrap method by sampling 90\% of the test data 100 times to calculate the standard deviation.}}
  \label{tbl:main_vwa}
\end{table}

==> floats/table_main_v2.tex <==

% \begin{table}[t!]
%   \centering
%   \scalebox{0.92}{
%   \begin{tabular}{lc ccc cc cc}
%     \toprule
%     \multirow{2}{*}{Method} & \multirow{2}{*}{Search} & \multirow{2}{*}{Value} & 
%     \multicolumn{2}{c}{Classifieds} & \multicolumn{2}{c}{Reddit} & \multicolumn{2}{c}{Shopping} \\
%     \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
%     & & & Tokens & Success & Tokens & Success & Tokens & Success\\
%     \midrule
%     % 53.8k/0.40k
%     \react{} & - & -
%     & 1x & 28.6\%
%     % 39.3k/0.48k
%     & 1x & 13.8\%
%     % 66.0k/0.46k
%     & 1x & 23.2\%\\
%     % ToT$_{\textrm{BFS}}$ & BFS
%     \tot{} & BFS & $\texttt{SA}$
%     % 151.1k/26.2k
%     & 3.2x & 30.7\% 
%     & 4.7x & 19.5\% 
%     % 195.8k/31.3k
%     & 4.3x & 29.2\% \\
%     % ToT$_{\textrm{DFS}}$ & DFS
%     \tot{} & DFS & $\texttt{SA}$
%     & 3.1x & 30.3\% 
%     % 148k/20.6k
%     & 4.2x & 16.7\% 
%     & 4.0x & 28.3\% \\
%     % Search Agent & A-star 
%     \searchagent & Best-First & $\texttt{SA}$
%     & 4.2x & 33.8\%
%     & 5.4x & 21.9\%
%     & 5.1x & 30.3\%\\
%     % mcts above + the prompt changes used in rmcts_v7.2
%     \mcts{} & MCTS & $\texttt{SA}$
%     % 350k/35k
%     & 7.2x & 37.6\%
%     & 9.5x & 23.8\% %
%     & 8.9x & 29.4\% \\%
%     \midrule
%     % reinforced policy + reinforced rubric value function
%     % +some policy prompt fixing25_classifields_0-75
%     \rmcts{} & MCTS & $\texttt{SA}$
%     % 332k/50k
%     & 7.3x & 40.2\%
%     % 300k/34k
%     & 7.3x & 25.2\%
%     % 332k/45k
%     & 7.6x & 31.9\%
%     \\
%     % reinforced policy + reinforced debate value function
%     \rmcts{} & MCTS  & $\texttt{MAD}$
%     % 373.6k/34.0k
%     & 7.4x & \textbf{41.0}\%
%     % 560k/37.7k
%     & 9.7x & \textbf{28.7}\%
%     % 674k/49.5k
%     & 10.1x & \textbf{32.3}\%
%     \\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Comparing different agent's token consumption and performance on VisualWebArena. We show average token used per task using \react{} as a baseline.}
%   \label{tbl:main_vwa}
% \end{table}


% \begin{table}[t!]
%   \centering
%   \scalebox{0.92}{
%   \begin{tabular}{lc ccc cc cc}
%     \toprule
%     \multirow{2}{*}{Method} & \multirow{2}{*}{Search} & \multirow{2}{*}{Value} & 
%     \multicolumn{2}{c}{Classifieds} & \multicolumn{2}{c}{Reddit} & \multicolumn{2}{c}{Shopping} \\
%     \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
%     & & & Tokens & Success & Tokens & Success & Tokens & Success\\
%     \midrule
%     % 53.8k/0.40k
%     \react{} & - & -
%     & 1x & 28.6\%
%     % 39.3k/0.48k
%     & 1x & 13.8\%
%     % 66.0k/0.46k
%     & 1x & 23.2\%\\
%     % ToT$_{\textrm{BFS}}$ & BFS
%     \tot{} & BFS & $\texttt{SA}$
%     % 151.1k/26.2k
%     & 3.2x & 30.7\% 
%     & 4.7x & 19.5\% 
%     % 195.8k/31.3k
%     & 4.3x & 29.2\% \\
%     % ToT$_{\textrm{DFS}}$ & DFS
%     \tot{} & DFS & $\texttt{SA}$
%     & 3.1x & 30.3\% 
%     % 148k/20.6k
%     & 4.2x & 16.7\% 
%     & 4.0x & 28.3\% \\
%     % Search Agent & A-star 
%     \searchagent & Best-First & $\texttt{SA}$
%     & 4.2x & 33.8\%
%     & 5.4x & 21.9\%
%     & 5.1x & 30.3\%\\
%     % mcts above + the prompt changes used in rmcts_v7.2
%     \mcts{} & MCTS & $\texttt{SA}$
%     % 350k/35k
%     & 7.2x & 37.6\%
%     & 9.5x & 23.8\% %
%     & 8.9x & 29.4\% \\%
%     \midrule
%     % reinforced policy + reinforced rubric value function
%     % +some policy prompt fixing25_classifields_0-75
%     \thinkact{} & R-MCTS & $\texttt{SA}$
%     % 332k/50k
%     & 7.3x & 40.2\%
%     % 300k/34k
%     & 7.3x & 25.2\%
%     % 332k/45k
%     & 7.6x & 31.9\%
%     \\
%     % reinforced policy + reinforced debate value function
%     \thinkact{} & R-MCTS & $\texttt{MAD}$
%     % 373.6k/34.0k
%     & 7.4x & \textbf{41.0}\%
%     % 560k/37.7k
%     & 9.7x & \textbf{28.7}\%
%     % 674k/49.5k
%     & 10.1x & \textbf{32.3}\%
%     \\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Comparing different agent's token consumption and performance on VisualWebArena. We show average token used per task using \react{} as a baseline.}
%   \label{tbl:main_vwa}
% \end{table}


\begin{table}[t!]
  \centering
  \scalebox{0.99}{
  \begin{tabular}{l ccc cc cc}
    \toprule
    \multirow{2}{*}{Search}  & \multirow{2}{*}{Value} & 
    \multicolumn{2}{c}{Classifieds} & \multicolumn{2}{c}{Reddit} & \multicolumn{2}{c}{Shopping} \\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
    & & Tokens & Success & Tokens & Success & Tokens & Success\\
    \midrule
    % data/visualwebarena/eval_results/cot_som/gpt-4o_v6.1_classifields_80_tsubset
    % 53.8k/0.40k
    \xmark \, (\react{}) & -
    & 1x & 28.6\%
    % data/visualwebarena/eval_results/cot_som/gpt-4o_v6_reddit_80_tsubset
    % 39.3k/0.48k
    & 1x & 13.8\%
    % data/visualwebarena/eval_results/cot_som/gpt-4o_v6.1_shopping_120_tsubset
    % data/visualwebarena/eval_results/cot_som/gpt-4o_v6.1_shopping_0-465
    % 66.0k/0.46k
    & 1x & 23.2\%\\
    % ToT$_{\textrm{BFS}}$ & BFS
    \tot{}$_\texttt{BFS}$ & $\texttt{SA}$
    % data/visualwebarena/eval_results/tot_som/gpt-4o_v6.1cached_bfs_vrubric_classifields_80_tsubset
    % 151.1k/26.2k
    & 3.2x & 30.7\% 
    & 4.7x & 19.5\% 
    % data/visualwebarena/eval_results/tot_som/gpt-4o_v6.1cached_vrubric_shopping_120_tsubset
    % 195.8k/31.3k
    & 4.3x & 29.2\% \\
    % ToT$_{\textrm{DFS}}$ & DFS
    \tot{}$_\texttt{DFS}$ & $\texttt{SA}$
    & 3.1x & 30.3\% 
    % 148k/20.6k
    & 4.2x & 16.7\% 
    & 4.0x & 28.3\% \\
    % Search Agent & A-star 
    \searchagent{} & $\texttt{SA}$
    % data/visualwebarena/eval_results/searchagent_som/gpt-4o_v6.1cached_classifields_80_tsubset
    & 4.2x & 33.8\%
    & 5.4x & 21.9\%
    & 5.1x & 30.3\%\\
    % mcts above + the prompt changes used in rmcts_v7.2
    MCTS & $\texttt{SA}$
    % 350k/35k
    & 7.2x & 37.6\%
    & 9.5x & 23.8\% %
    & 8.9x & 29.4\% \\%
    \midrule
    % reinforced policy + reinforced rubric value function
    % +some policy prompt fixing25_classifields_0-75
    \rmcts{} & $\texttt{SA}$
    % data/visualwebarena/eval_results/rmcts_som/gpt-4o_v7.2cached_refl3_vrubric_classifields_80_tsubset
    % 332k/50k
    & 7.3x & 40.2\%
    % 300k/34k
    & 7.3x & 25.2\%
    % 332k/45k
    & 7.6x & 31.9\%
    \\
    % reinforced policy + reinforced debate value function
    \rmcts{}  & $\texttt{MAD}$
    % data/visualwebarena/eval_results/rmcts_som/gpt-4o_v7.4.1cached_refl3_vredebate_trhld0.5_classifields_80_tsubset
    % 373.6k/34.0k
    & 7.4x & \textbf{41.0}\%
    % data/visualwebarena/eval_results/rmcts_som/gpt-4o_v7.4.1cached_refl3_vredebate_trhld0.5_reddit_80_tsubset
    % 560k/37.7k
    & 9.7x & \textbf{28.7}\%
    % 674k/49.5k
    & 10.1x & \textbf{32.3}\%
    \\
    \bottomrule
  \end{tabular}
  }
  \caption{Comparing different agent's token consumption and performance on VisualWebArena. We show average token used per task using \react{} as a baseline.}
  \label{tbl:main_vwa}
\end{table}

==> floats/table_test_time_compute.tex <==
\begin{table}[h]
  \centering
  \begin{tabular}{llcccc}
    \toprule
    Method & Model & \#Node & Tokens & Success Rate\\
    \midrule
    % Search Agent & GPT-4o & 5 & 167k & 31.2\%\\
    % Search Agent & GPT-4o & 15 & 231k & 36.3\%\\
    % % breath = 10
    % Search Agent & GPT-4o & 30 & r & r\%\\
    % \midrule
    ReAct & GPT-4o & - & 54k & 28.6\%\\
    \rmctsdebate{} & GPT-4o & 2 & 220k & 35.0\%\\
    \rmctsdebate{} & GPT-4o & 5 & 420k & 37.6\%\\
    \rmctsdebate{} & GPT-4o & 10 & 579k & 43.6\%\\
    % breath 7
    \rmctsdebate{} & GPT-4o & 15 & 690k & 47.5\%\\
    \bottomrule
  \end{tabular}
  \caption{Inference time scaling with classifields}
  \label{tbl:inference_time_scaling_main}
\end{table}
